Active inference for action-unaware agents

Active inference is a formal approach to study cognition based on the notion that adaptive agents can be seen as engaging in a process of approximate Bayesian inference, via the minimisation of variational and expected free energies. Minimising the former provides an account of perceptual processes and learning as evidence accumulation, while minimising the latter describes how agents select their actions over time. In this way, adaptive agents are able to maximise the likelihood of preferred observations or states, given a generative model of the environment. In the literature, however, different strategies have been proposed to describe how agents can plan their future actions. While they all share the notion that some kind of expected free energy offers an appropriate way to score policies, sequences of actions, in terms of their desirability, there are different ways to consider the contribution of past motor experience to the agent's future behaviour. In some approaches, agents are assumed to know their own actions, and use such knowledge to better plan for the future. In other approaches, agents are unaware of their actions, and must infer their motor behaviour from recent observations in order to plan for the future. This difference reflects a standard point of departure in two leading frameworks in motor control based on the presence, or not, of an efference copy signal representing knowledge about an agent's own actions. In this work we compare the performances of action-aware and action-unaware agents in two navigations tasks, showing how action-unaware agents can achieve performances comparable to action-aware ones while at a severe disadvantage.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%
% Adjusted and extended from https://github.com/goodfeli/dlbook_notation.

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}

% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
%\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\DeclarePairedDelimiterX{\infdivx}[2]{(}{)}{%
	#1\;\delimsize\|\;#2%
}
\newcommand{\infdiv}{\KL \infdivx}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

%%%% Commands below added by Filippo Torresan and Manuel Baltieri %%%%
% In-text comments
\newcommand{\comm}[1]{\textcolor{OrangeRed}{[#1]}}
% Definitions, Propositions, Principles, and Theorems (all requiring amsthm)
% Definition
\theoremstyle{definition}
\newtheorem{definition}{Definition}[section]
\theoremstyle{plain}
\newtheorem{proposition}{Proposition}[section]
\theoremstyle{plain}
\newtheorem{principle}{Principle}[section]
\theoremstyle{plain}
\newtheorem{theorem}{Theorem}[section]
\theoremstyle{definition}
\newtheorem{remark}{Remark}[section]
\tcolorboxenvironment{remark}{colframe=ForestGreen,breakable,before skip=10pt,after skip=10pt}

\newtheorem{example}[theorem]{Example}



\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

% For argmax and argmin operators
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

% For probabilistic independence and dependence symbols
\newcommand{\indep}{\perp\!\!\!\!\perp}
\newcommand{\nindep}{\centernot{\indep}}

% backward blocking
\newcommand{\CueOne}{\mathbf{C}_1}
\newcommand{\CueTwo}{\mathbf{C}_2}
\newcommand{\Outcome}{\mathbf{+}}

% maths
\newcommand{\N}{\mathbb{N}}
\newcommand{\id}{\mathsf{id}}
\newcommand{\card}[1]{\lvert{#1}\rvert}
\newcommand{\prob}[1]{P(#1)}
\newcommand{\condprob}[2]{P({#1}|{#2})}
\newcommand{\definedas}{\doteq}

% POMDP
\newcommand{\statespace}{\mathcal{S}}
\newcommand{\obsspace}{\mathcal{O}}
\newcommand{\actionspace}{\mathcal{A}}
\newcommand{\policyspace}{\Pi}
\newcommand{\Transition}{\mathcal{T}}
\newcommand{\Emission}{\mathcal{E}}
\newcommand{\ntime}{T}
\newcommand{\horizon}{H}
\newcommand{\action}{a}
\newcommand{\ohaction}{\mathbf{\mathsf{a}}}
\newcommand{\actionvar}{A}
\newcommand{\state}{s}
\newcommand{\ohstate}{\mathbf{\mathsf{s}}}
\newcommand{\statevar}{S}
\newcommand{\obs}{o}
\newcommand{\ohobs}{\mathbf{\mathsf{o}}}
\newcommand{\obsvar}{O}
\newcommand{\tprob}[1]{P({#1}| \state_{t}, \action_{t})}
\newcommand{\eprob}[1]{P({#1}| \state_{t})}

% Active inference
\newcommand{\fe}{\mathcal{F}}
\newcommand{\efe}{\mathcal{G}}
\newcommand{\totefe}{\mathcal{G}_{\polhorizon}}
\newcommand{\kldiv}{\mathcal{D}_{KL}}
\newcommand{\pprob}[1]{P^{*}({#1})}
\newcommand{\stateparams}{\mathbf{s}}
\newcommand{\obsparams}{\mathbf{o}}
\newcommand{\policyparams}{\boldsymbol{\policy}}
\newcommand{\seqstates}[1]{\state_{1}, \dots, \state_{{#1}}}
\newcommand{\seqobs}[1]{\obs_{1}, \dots, \obs_{{#1}}}
\newcommand{\seqactions}[1]{\action_{1}, \dots, \action_{{#1}}}
\newcommand{\decision}{d}
\newcommand{\genmodel}{\mathcal{M}}
\newcommand{\gmparams}{\boldsymbol{\Theta}}
\newcommand{\varapprox}{\mathcal{V}}
\newcommand{\seqv}[3]{{#1}_{#2:#3}}
\newcommand{\policy}{\pi}
\newcommand{\polhorizon}{H}
\newcommand{\numpolicies}{\mathtt{p}}
\newcommand{\obsmap}{\mathbf{A}}
\newcommand{\transmap}{\mathbf{B}}
\newcommand{\tprobaif}{P(\statevar_{t}| \statevar_{t-1}, \policy, \transmap)}
\newcommand{\eprobaif}{P(\obsvar_{t}| \statevar_{t-1}, \obsmap)}
\newcommand{\varprob}[1]{Q(#1)}
\newcommand{\softmax}[1]{\sigma(#1)}
\newcommand{\entropy}{\mathbb{H}}

% RL
\newcommand{\actions}{\mathbf{a}}
\newcommand{\Actions}{A}
\newcommand{\reward}{r}
\newcommand{\Reward}{R}
\newcommand{\Reals}{\mathbb{R}}
\newcommand{\Observations}{M}
\newcommand{\stateaction}{\tau}
\newcommand{\obsaction}{\tau^{\text{POMDP}}}
\newcommand{\policyparameters}{{\boldsymbol{\theta}}}
\newcommand{\Advantage}{\text{Adv}}
\newcommand{\return}{G}
\newcommand{\expreturn}{J}
\newcommand{\valuefunction}{V}
\newcommand{\beliefs}{B}

% actor-critic
\newcommand{\behavioural}{{\boldsymbol{\beta}}}
\newcommand{\importanceweights}{{\boldsymbol{w}_{T}^{i}}}
\newcommand{\discount}{\gamma}
\newcommand{\estexpreturn}{\hat{\expreturn}}
\newcommand{\Qfunction}{Q}
\newcommand{\ntrajectories}{N}

\newcommand{\itertrajectories}{n}
\newcommand{\itertime}{t}
\newcommand{\iterpartial}{i}

% scm
\newcommand{\noise}{N}
\newcommand{\scm}{\mathcal{C}}
\newcommand{\assignment}{h}
\newcommand{\emission}{g}
\newcommand{\PA}{\mathbf{PA}}

\newcommand{\confounders}{\mathbf{c}}
\newcommand{\Confounders}{C}
\newcommand{\nconfounders}{m}


% autoencoder
\newcommand{\Data}{\mathcal{D}}
\newcommand{\encoderweights}{\boldsymbol{\phi}}
\newcommand{\decoderweights}{\boldsymbol{\theta}}
\newcommand{\ELBO}{\mathcal{L}}
\newcommand{\VAELoss}{\ELBO}


%*********************************************************************************
% Listings Settings
%*********************************************************************************

% Setting the format for all the codes in line and float objects with \lstset
\lstset{language=Python,
	keywordstyle=\color{Plum},%\bfseries,
	basicstyle=\normalsize \ttfamily,
	identifierstyle=\color{Black},
	commentstyle=\color{Gray}\ttfamily,
	stringstyle= \color{LimeGreen} \rmfamily,
	numbers=left,%left,%
	numberstyle=\scriptsize, %\tiny %
	stepnumber=1,
	numbersep=8pt,
	%showstringspaces=false,
	%breaklines=true,
	%frameround=ftff,
	frame=single,
	%backgroundcolor = \color{},
	keepspaces=true
}

% Custom environment for all the codes in display in Python
\lstnewenvironment{Python}{\lstset{language=Python,
		keywordstyle=\color{Plum},%\bfseries,
		basicstyle=\small \ttfamily,
		identifierstyle=\color{Black},
		commentstyle=\color{Gray}\ttfamily,
		stringstyle= \color{LimeGreen} \rmfamily,
		numbers=left,%left,%
		numberstyle=\scriptsize, %\tiny
		stepnumber=1,
		numbersep=8pt,
		%showstringspaces=false,
		%breaklines=true,
		%frameround=ftff,
		frame=none,
		%backgroundcolor = \color{},
		keepspaces=true
	}}{}

% new listing object with tcolorbox package
\newtcblisting[auto counter, number within=section]{code}[2][]{
	fonttitle=\bfseries, colback=black!5!white, colframe=black!73!white, listing only,
	listing options={
			language=Python,
			keywordstyle=\color{Plum},%\bfseries,
			basicstyle=\normalsize \ttfamily,
			identifierstyle=\color{Black},
			commentstyle=\color{Gray}\ttfamily,
			stringstyle= \color{LimeGreen} \rmfamily,
			numbers=left,%left,%
			numberstyle=\scriptsize, %\tiny
			stepnumber=1,
			numbersep=8pt,
			%showstringspaces=false,
			%breaklines=true,
			%frameround=ftff,
			frame=none,
			%backgroundcolor = \color{},
			keepspaces=true},
	title=Code \thetcbcounter: #2, #1}

% new tcolorbox object for pseudocode with algorithm2e
% Argument #2 corresponds to the title for the box, argument #1 is optional and will add a label if given
% Example: \begin{pscode}[label={pscode:aaa}]{Pscode One}

\newtcolorbox[use counter=pscode, list inside = boxes]{pscode}[2][]{
	fonttitle=\bfseries,
	colback=black!5!white,
	colframe=black!73!white,
	before upper={\begin{algorithm}[H]},
				after upper={\end{algorithm}},
	%floatplacement=tb, float,
	title=Algorithm \thepscode: #2, #1}

% Define the counter to avoid "! LaTeX Error: No counter 'pscode' defined." when the counter is not
% automatically created, e.g., because there are no pscode environments in the main texts, triggering
% the error when we use \setcounter{pscode}{0} (but no counter exists) as part of \beginsupplement (see araya.csl)
\newcounter{pscode}
\crefname{pscode}{Algorithm}{Algorithms}
\Crefname{pscode}{Algorithm}{Algorithms}


% Example LaTeX code (to be copied and modified for a specific case)
%\begin{pscode}[label={pscode:perc-inf}]{Perceptual Inference}
%  \DontPrintSemicolon
%  \KwData{sensory observations, i.e.\ $o_{1}, \dots, o_{t}$, and policies $\pi_{1} \dots \pi_{n}$.}
%  \KwResult{updated beliefs about the states, i.e.\ $Q(S_{1}|\pi), \dots, Q(S_{T}|\pi)$.}
%  \BlankLine
%  \For{$\pi_{i} \in [\pi_{1} \dots \pi_{n}]$}{
%    \While{$ \mathcal{F}_{\pi_{i}} > \epsilon$}{
%      \For{$t \in [1 \dots T]$}
%      {$\mathbf{s}^{\pi_{i}}_{t} := \mathbf{s}^{\pi_{i}}_{t} - \nabla_{\mathbf{s}^{\pi_{i}}_{t}} \mathcal{F}_{\pi_{i}}$}
%    }}
%\end{pscode}

% new theorem box with tcolorbox package
\newtcbtheorem[auto counter, number within=section, list inside = boxes]{mytheo}{My Theorem}%
{colback=green!5,colframe=green!35!black,fonttitle=\bfseries}{th}

